CSS Minification via Constraint Solving (Technical Report)

Minification is a widely-accepted technique which aims at reducing the size of the code transmitted over the web. We study the problem of minifying Cascading Style Sheets (CSS) --- the de facto language for styling web documents. Traditionally, CSS minifiers focus on simple syntactic transformations (e.g. shortening colour names). In this paper, we propose a new minification method based on merging similar rules in a CSS file. We consider safe transformations of CSS files, which preserve the semantics of the CSS file. The semantics of CSS files are sensitive to the ordering of rules in the file. To automatically identify a rule merging opportunity that best minimises file size, we reduce the rule-merging problem to a problem on CSS-graphs, i.e., node-weighted bipartite graphs with a dependency ordering on the edges, where weights capture the number of characters (e.g. in a selector or in a property declaration). Roughly speaking, the corresponding CSS-graph problem concerns minimising the total weight of a sequence of bicliques (complete bipartite subgraphs) that covers the CSS-graph and respects the edge order. We provide the first full formalisation of CSS3 selectors and reduce dependency detection to satisfiability of quantifier-free integer linear arithmetic, for which highly-optimised SMT-solvers are available. To solve the above NP-hard graph optimisation problem, we show how Max-SAT solvers can be effectively employed. We have implemented our algorithms using Max-SAT and SMT-solvers as backends, and tested against approximately 70 real-world examples (including the top 20 most popular websites). In our benchmarks, our tool yields larger savings than six well-known minifiers (which do not perform rule-merging, but support many other optimisations). Our experiments also suggest that better savings can be achieved in combination with one of these six minifiers.

==> abstract.tex <==
In the web programming literature, minification is a widely-accepted
technique which aims at reducing the size of the code transmitted
over the web.
This paper
concerns the problem of minifying Cascading Style Sheets (CSS) ---
the de facto language for styling web documents.
Traditionally, CSS minifiers focus on simple syntactic
transformations (e.g. shortening colour names). 
In this paper, we propose a new minification method based on 
merging similar rules in a CSS file.

This work considers safe transformations of CSS files, which preserve the 
semantics 
of the CSS file (i.e. style any document tree in the same way). The cascading
nature of CSS makes the semantics of CSS files sensitive to the ordering of 
rules in the file.
To automatically identify a rule merging opportunity that best minimise
file size, we
reduce the rule-merging problem to a problem concerning CSS-graphs, i.e., 
node-weighted 
bipartite graphs with a dependency ordering on the edges, where weights 
capture the number of characters (e.g. in a selector or in a property
declaration). Roughly speaking, the corresponding CSS-graph problem concerns
minimising the total weight of a sequence of bicliques (complete bipartite 
subgraphs) that covers the CSS-graph and respects the edge order.


Constraint solving plays a key role in both our transformation from a CSS
file to a CSS-graph, and our algorithm for solving the NP-hard optimisation
problem of CSS-graphs.
The former problem requires us to extract the dependency ordering on the edges 
of a CSS-graph (an NP-hard problem), which requires us to solve
the selector intersection problem (i.e. check whether two given selectors may 
match the same node in some document tree). To solve the selector intersection
problem, we provide the first full formalisation of CSS3 selectors (the most 
stable version of CSS) and reduce their selector intersection problem
to satisfiability of quantifier-free integer linear arithmetic, for which 
highly-optimised SMT-solvers are available. To solve the above NP-hard
graph optimisation problem, 
we show how Max-SAT solvers can be effectively employed. 
We have implemented our rule merging algorithm using Max-SAT and 
SMT-solvers as backends, 
and tested our tool against approximately $70$ real-world examples (including
those from the top 20 most popular websites listed on Alexa). 
In our benchmarks, we found that our tool (which only performs refactoring) 
yields larger
savings than six well-known minifiers (which do not perform rule-merging, but
support many other optimisations). Our experiments also suggest that
an even larger overall savings can be achieved if we apply our tool
after first applying one of these six minifiers.


==> conc.tex <==
HARKHARK


\section{Conclusion}
\label{sec:conc}
In this paper, we have provided an algorithm for performing CSS
refactoring by means of merging and combining similar rules in a given
CSS file, and apply it to the problem of CSS minification. A crucial property
of our algorithm is that it discovers the best refactoring opportunity (i.e.
that best minimises the file size) while preserving the semantics of the
original CSS file. Precise mechanised formalisation of CSS3 selectors
(in quantifier-free integer linear arithmetic) and the use of SMT/Max-SAT
solvers are paramount for our algorithm.

We now mention some future work.
As we mentioned, merging and combining rules in a CSS file is only one
among many CSS minification opportunities. So far, we have crudely combined
cssnano and our tool in our study. We have discovered that
cssnano can be applied before and after running our tool to produce
further space saving.
\begin{future}
Fully integrate our refactoring technique with existing
minification techniques to provide the best possible minification.
\end{future}
We also
leave it for future work to optimise our method so as to provide the best
file size reduction \emph{after gzip compression}.
[Gzip is now supported by many web hosts and most modern browsers (not including
old IE browsers).] A systematic study of which CSS minification
techniques are effective after gzip compression is still lacking and deserves
a serious attention in the CSS minification community, especially since some
CSS minification techniques might actually \emph{enlarge} the file size after
compression. One simple technique that could help bring down the compressed
file size is to sort the selectors and declarations in each rule after the
minification process is done \cite{advanced-css-book}. To perform this
sorting without changing the order-dependency (and hence the semantics) of the
original CSS file, one actually has to be a bit careful when sorting the
declarations (many off-the-shelf declaration sorters often use ordering of
declarations that could change the semantics of the original CSS file).
Therefore, a specific research question is:
\begin{future}
Find a safe ordering of
declarations that could provide the best minification result after compression.
\end{future}
A simple ordering of declarations is
%stable sorting
%algorithms with
to first apply the alphabetical ordering after applying the key function that
maps related property names (including
shorthands) to the same value. %, and then apply alphabetical order.
A stable algorithm with this key function results in a safe sorting of
declarations. Using this ordering (both after running
cssnano and running our tool), preliminary studies show that, if we apply
cssnano
before and after applying our tool, the resulting CSS files after gzip
compression are typically smaller by 70--300 Bytes (in our examples) than
performing cssnano without applying our tool. [One exception is the amazon.css
example, where this actually results in a bigger gzip file.] Although these
numbers
sound comparatively small, %it has not escaped our attention that
the impact on the bandwidth for a
web page with a large number of visitors (e.g. close to 3 Billion per month
as in the case of Amazon.com) could be non-negligible.

